Joint Optimal Pricing and Electrical Efficiency Enforcement for Rational Agents in Micro Grids

In electrical distribution grids, the constantly increasing number of power generation devices based on renewables demands a transition from a centralized to a distributed generation paradigm. In fact, power injection from Distributed Energy Resources (DERs) can be selectively controlled to achieve other objectives beyond supporting loads, such as the minimization of the power losses along the distribution lines and the subsequent increase of the grid hosting capacity. However, these technical achievements are only possible if alongside electrical optimization schemes, a suitable market model is set up to promote cooperation from the end users. In contrast with the existing literature, where energy trading and electrical optimization of the grid are often treated separately or the trading strategy is tailored to a specific electrical optimization objective, in this work we consider their joint optimization. Specifically, we present a multi-objective optimization problem accounting for energy trading, where: 1) DERs try to maximize their profit, resulting from selling their surplus energy, 2) the loads try to minimize their expense, and 3) the main power supplier aims at maximizing the electrical grid efficiency through a suitable discount policy. This optimization problem is proved to be non convex, and an equivalent convex formulation is derived. Centralized solutions are discussed first, and are subsequently distributed. Numerical results to demonstrate the effectiveness of the so obtained optimal policies are then presented.

==> IEEEtran/README <==

December 27, 2012


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.8 is a significant update over the 1.7a release. For a full list of
changes, please read the file changelog.txt. The most notable changes
include:


 1) New transmag class option to support the IEEE Transactions on Magnetics
    format. Thanks to Wei Yingkang, Sangmin Suh and Benjamin Gaussens
    for suggestions and beta testing.

 2) The \IEEEcompsoctitleabstractindextext and 
    \IEEEdisplaynotcompsoctitleabstractindextext
    commands have been deprecated in favor of their
    \IEEEtitleabstractindextext and \IEEEdisplaynontitleabstractindextext
    (observe that the "not" has changed to "non") equivalents. This change
    generalizes and decouples them from compsoc mode because the new
    transmag mode also uses them now.

 3) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.
 
 4) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 5) Revised spacing at top of top figures and tables to better
    align with the top main text lines as IEEE does in its journals. 
    Thanks to Dirk Beyer for reporting this issue and beta testing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> scenario_extended.tex <==
%!TEX root = main.tex
In this section, the electrical, communication and market scenarios are introduced. \revision{Some relevant use cases are described, showing how two electrical optimization techniques from the literature can be plugged into the proposed optimization framework. In particular, we define the communication requirements and infrastructure needed to support the proposed model and discuss the  interactions among the involved (rational) agents.}

\subsection{Electrical Scenario}
\label{ssec:cap_5_electrical_scenario}

\begin{figure}[t]
\begin{center}
\def\svgwidth{0.45\textwidth}
\input{./figures/grid-opt.eps_tex}
\end{center}
\caption{Electrical network example, where $B_i,\ i=1,\dots,4$ are the electrical distribution lines, $L_j,\ j=1,2$ are the loads, $G_k,\ k=1,2$ are the DERs, and the PCC is the Point of Common Coupling.}
\label{figure:cap_5_electrical_network}
\end{figure}

We consider a steady-state\footnote{In steady-state, the network has reached equilibrium and transient phenomena are no longer relevant.} low voltage power micro grid. For \revision{ease of computation}, and without loss of generality, the considered grid is modeled as a directed tree. The root of the tree represents the Point of Common Coupling (PCC) and the other nodes represent loads and Distributed Energy Resources (DERs). Loads are either \revision{modeled} by constant complex impedances or by constant current sources, the PCC is modeled as a voltage generator setting the voltage \revision{and phase} references for the entire grid, while DERs are modeled either as power or current generators. \revision{Here, we assume that the PCC is always able to supply the grid with the needed power. Hence, no power outages or voltage instabilities (i.e., overvoltages and voltage sags due to the DERs operations) can occur in the considered electrical setup.} This model has been widely considered in the literature, and in particular for power loss minimization algorithms~\cite{TokenRing,SurroundControl,dyngridmap, DORPF,DORPFConvergence}.

\fig{figure:cap_5_electrical_network} \revision{shows} an example power grid is shown. DER $i=1,2$ and load $j=1,2$ are respectively denoted by $G_i$ and $L_j$. Distribution lines are assumed to have a constant section~\cite{SurroundControl, DORPF}, and hence each line has a constant impedance per unit length. The length of the $z$-th distribution line is denoted by $B_z$. Each DER is equipped with a finite-size energy storage device (e.g., rechargeable battery). The size of the energy storage devices determines the total amount of available power. Moreover, each DER is assumed to be feeding an associated load and to have the capability of injecting part of its energy surplus into the grid. The surplus power that DER $G_i$ can inject into the grid is denoted by $E_i$. For the sake of terminology, the quantity $E_i$ will be referred to as $G_i$'s surplus energy. \revision{The amount of energy $E_i$ that each DER wishes to inject into the grid is not regulated by a central authority, but it depends on its local decision. This decision, in turn, depends on the specific energy storage policy that each DER implements, as, for example, the minimization of the probability of not being able to feed its associated load within a given time horizon.} In this paper, it is assumed, without loss of generality, that $E_i\geq0\ \forall \, i$. Each load $L_j$ is assumed to have a non-negative power demand, which is denoted by $D_j \geq 0$. These assumptions are common in the literature, see for example~\cite{ICIT,DORPF,LC,TokenRing}.

%It is worth noting that the proposed model is not tailored to a specific (electrical) grid optimization strategy as long as it deals with the selection of the amount of power that each DER must inject into the grid to boost its electrical efficiency.

%is transparent with respect to the selected (electrical) grid optimization strategy as long as it deals with the selection of the amount of power that each DER must inject into the grid to boost its electrical efficiency.

\subsection{Communication Scenario}
\label{ssec:cap_5_comm_scenario}

Each node (i.e., loads, DERs and the PCC) in the grid is equipped with a transceiver, whose communication performance  depends on the requirements of the selected electrical optimization technique. These details are however neither considered here nor fundamental to the solution of the presented optimization problem. In fact, our optimization framework is independent of the specific  communication technology and infrastructure, as long as these allow a timely bi-directional communication between each pair of nodes.

\subsection{Market Scenario}
\label{ssec:cap_5_market_scenario}

We propose a market scenario where each DER can either sell its surplus power to the PCC or directly to the loads. The monetary revenue that each DER obtains by selling (part of) its energy to the PCC is determined by a PCC-imposed unitary {\it buying price}. The monetary revenue that each DER obtains by selling its energy directly to a specific load is determined by a DER-imposed unitary {\it selling price}. Each DER can independently set a different selling price for each load, i.e., this price is not controlled by the PCC. Also, each load can fulfill its power demand by buying the needed power from the PCC or directly from the DERs. DERs and loads are assumed to behave as {\it rational agents}. That is, each DER will sell its power to the agents (PCC and loads) ensuring the highest revenue, while each load will buy the power it needs from the agents (PCC and DERs) ensuring the lowest expense. Note that this trading model is consistent with the expected evolution of the smart grid market~\cite{PowerToPeople-2014}.

\begin{figure}[tbp]
\begin{center}
\unitlength=1mm
\begin{picture}(82,58)(0,0)
%\put(0,0){\framebox(82,58){}} %framebox to see actual figure size - very useful (uncomment) when creating the composition
%\w(80,92)[12]{\textbf{weekends:}}
\put(0,0){\includegraphics[width=0.48\columnwidth]{figures/price.eps}}
\w(17,44)[12]{PCC buying price: $\gamma_{i}^{\text{PCC}}$}
\w(65,44)[12]{PCC selling price: $\pi_{j}^{\text{PCC}}$}
\w(70,39)[12]{Discount: $\Sel{j}{i}$}
\w(40,21)[12]{Energy price: $\Pel{i}{j}$}
\w(40,50)[10]{PCC}
\w(17,25)[10]{$G_i$}
\w(18,14)[10]{DER $i$}
\w(64,14)[10]{Load $j$}
\w(63,25)[10]{$L_j$}
%\w(126,30)[12]{$w_3$}
%\w(135,30)[12]{$w_4$}
\end{picture}
\end{center}
\caption{Market scenario example. Here, the PCC can buy energy from DER $G_i$ paying unitary price $\gamma_i^{\text{PCC}}$, and it can sell energy to load $L_j$ for a unitary price $\pi_j^{\text{PCC}}$. Moreover, $L_j$ can buy energy from $G_i$ paying a discounted unitary price $\Pel{i}{j}-\Sel{j}{i}$, where the discount $\Sel{j}{i}$ is imposed by the PCC.}
\label{figure:cap_5_market_scenario}
\end{figure}


%\begin{figure}[h!]
%\begin{center}
%\def\svgwidth{0.4\textwidth}
%\input{./figures/scenario-opt.eps_tex}
%\end{center}
%\caption{Market scenario example.}
%\label{figure:cap_5_market_scenario}
%\end{figure}

\fig{figure:cap_5_market_scenario} shows an example for the considered market scenario. On the one hand, for each DER $G_i$, the PCC determines the unitary price $\gamma_{i}^{\text{PCC}}$. This is the unitary price that the PCC pays when buying power from DER $G_i$. On the other hand, for each load $L_j$ the PCC determines the unitary price $\pi_{j}^{\text{PCC}}$. This is the unitary price that load $L_j$ pays when buying power from the PCC. \revision{The prices $\gamma_i^{\text{PCC}}$ and $\pi_j^{\text{PCC}}$ do not depend on the optimization process. They are imposed by the PCC according to existing energy trading contracts. Each network agent may have different contract terms and conditions for buying and selling energy from and to the PCC. These conditions set the baseline for the proposed optimization to determine the new trading strategy. With respect to the current practice, where each DER sells $E_i$ energy to the PCC for $\gamma_i^{\text{PCC}}$ revenue and each load buys $D_j$ energy from the PCC spending $\pi_j^{\text{PCC}}D_j$, the new trading strategy results in economic benefits for the network agents, while also enforcing the  electric optimization policy already in place. In the proposed market model,} each DER $G_i$ proposes a unitary price $\Pel{i}{j}$ to each load $L_j$. The unitary price $\Pel{i}{j}$ determines the monetary revenue that $G_i$ obtains when selling power to $L_j$. In order to move the grid electrical state toward the optimal solution (dictated by the selected electrical grid optimization technique), the PCC can apply a discount to the unitary prices $\Pel{i}{j}$ proposed by the DERs to the loads. The discount proposed by the PCC to $L_j$ when buying from $G_i$ is denoted by $\Sel{j}{i}$ and, in turn, the unitary price that $L_j$ pays to $G_i$ is $\Pel{i}{j}-\Sel{j}{i}$. Similar interaction models have been previously used in the scientific literature see, e.g.,~\cite{Pricing-2015}. \revision{We remark that, since DERs and loads are assumed to be {\it rational} agents, any energy trading solution resulting in higher revenues for the DERs and in lower expenses for the loads with respect to the current practice will be embraced. Here, we propose an optimization problem whose solution guarantees better trading conditions for DERs and loads with respect to the current energy trading paradigm and, at the same time, enforces the operation of an electrical optimization technique that is possibly already in place. With respect to the current energy market, the only regulatory act to enable the proposed optimized market is to allow direct energy trading between the grid agents. As noted before, this scenario is expected to become a solid reality in the near future.}

To optimize the electrical status of the power network, we allow the PCC to influence the amount of energy that the DERs inject into the grid. In particular, PCC can prevent DERs from injecting energy by buying it. In this case, the energy bought by the PCC is for example stored by the DERs into their batteries, and could be made available for future use. 

%In the proposed model, the amount of power that $G_i$ sells to the PCC is not injected into the grid. It is, instead, stored into $G_i$'s battery assuming that, at any time, the PCC can claim its ownership and, in turn, force $G_i$ to inject a fraction of that power into the grid. This assumption is needed so that the PCC can buy power from the DERs while, at the same time, enforcing the electrical grid's efficiency. In fact, if the DERs would inject into the grid the power they sell to the PCC, then all the available power would always be injected into the grid, making any optimization of its electrical status impossible.

%All the assumptions and motivation of this section are coherent with standard assumptions and motivation in the literature (CITA). In the following section, the needed mathematical notation will be introduced.

\subsection{Use Cases}
\revision{\myparstart{i) }In the first use case, we consider the current based surround control (CBSC) proposed in~\cite{SurroundControl}. When this technique is implemented, the electrical network is divided into clusters. Each cluster is made of a pair of DERs connected such as on the path between them there are only loads. Within each cluster, the DERs cooperate to feed the loads on the path connecting them. The framework proposed in this paper can be utilized to enforce CBSC by defining market rules that guarantee economic advantages for the loads and the DERs. First, the DERs in each cluster have to solve an electrical optimization problem. To do that, the DERs collect the amount of power needed by the loads. Then, they determine the optimal amount of power that they should inject into the grid to minimize the distribution losses as described in~\cite{SurroundControl}. Once this process is complete, the DERs send to the PCC the information they obtained (i.e., the optimal amount of power that they should inject and the power needed by the loads) together with the maximum amount of power they are willing to sell (i.e., to inject). The PCC collects this information and, by solving the optimization problem defined in this paper determines the prices $p_{i,j}$ and the discounts $s_{j,i}$ of~\fig{figure:cap_5_market_scenario} which guarantee that, when acting as rational agents, DERs and loads experience economic benefits while minimizing the grid power losses. This process can be carried out according to different time scales (i.e., real time, on a minute basis, or on an hourly basis), moreover the electrical optimization time scale and the market one can be decoupled. For example, the electrical optimization can operate in real time, while the market one can operate on an hourly basis. In this case, DERs and loads must send to the PCC hourly generation and consumption data. This can be done in a day ahead fashion by forecasting the power generation and consumption of the next hour in each cluster. This information is then sent to the PCC, who solves the electrical optimization problem assuming a constant power consumption and generation during the next hour and determines the prices $p_{i,j}$ and the discounts $s_{j,i}$ to be applied accordingly. Once this is done, the electrical optimization is performed in real time, but the energy trading strategy remain the same until the next update of market quantities (prices).}

\revision{\myparstart{ii) } The second use case deals with the peak shaving technique in~\cite{ICIT}. This optimization requires that the DERs send to the PCC a day ahead forecast of the generated power. Once the PCC receives this information, it performs a day ahead forecast of the grid power consumption and, based on these two predictions, it computes two parameters that are broadcast to the DERs. Once they receive these parameters, the DERs determine the amount of active and reactive power that they will inject into the grid. Differently from CBSC, in this case only the aggregated power consumption from the loads is required. Nevertheless, the computation of a suitable trading strategy, through the optimization that we propose in this paper, requires one to know the power consumption of {\it each} load. According to the growing diffusion of home deployed smart meters~\cite{SMART-METERS}, this fine-grained information is easily gathered and is expected to be available in nearly all future power grids. With this information, it is possible to perform the market optimization proposed here. To do that, the PCC determines the optimal amount of power that the DERs have to generate to prevent power consumption peaks. Moreover, it determines the amount of power that the DERs have to sell to the loads to fulfill their power demand. For example, consider~\fig{figure:cap_5_electrical_network} and assume that the electrical optimization process dictates that DERs $G_1$ and $G_2$ inject $E_1$ and $E_2$ power, respectively. Moreover, assume that loads $L_1$ and $L_2$ will need $D_1$ and $D_2$ power, respectively. Then, a possible power allocation scheme could be:
\begin{itemize} 
\item $\min(E_1,D_1)$ power is sold by $G_1$ to $D_1$;
\item $\min(E_2,D_2)$ power is sold by $G_2$ to $D_2$;
\item the remaining available (needed) power is sold to (bought from) the PCC.
\end{itemize}
This information is then sent to the DERs and loads, respectively. After that, the PCC solves the optimization problem presented here, obtaining the prices $p_{i,j}$ and discounts $s_{j,i}$ of~\fig{figure:cap_5_market_scenario}.
As in the previous case, different time scales can be used for the electrical and market optimization processes.}
